Test case generation for agent-based models: A systematic literature review

Agent-based models play an important role in simulating complex emergent phenomena and supporting critical decisions. In this context, a software fault may result in poorly informed decisions that lead to disastrous consequences. The ability to rigorously test these models is therefore essential. In this systematic literature review, we answer five research questions related to the key aspects of test case generation in agent-based models: What are the information artifacts used to generate tests? How are these tests generated? How is a verdict assigned to a generated test? How is the adequacy of a generated test suite measured? What level of abstraction of an agent-based model is targeted by a generated test? Our results show that whilst the majority of techniques are effective for testing functional requirements at the agent and integration levels of abstraction, there are comparatively few techniques capable of testing society-level behaviour. Additionally, we identify a need for more thorough evaluation using realistic case studies that feature challenging properties associated with a typical agent-based model.

==> sections/__latexindent_temp.tex <==
\section{Introduction}
In recent years, computational models have become increasingly popular in a variety of domains, with applications ranging from economic modelling \cite{liu2020interbank} to public health \cite{tracy2018agent}. The ability to model and understand vast quantities of data, coupled with the increased availability of data, have helped to establish the computational model as an essential research tool. Agent-based models are one variety of computational model that are used to simulate complex scenarios involving many individuals, often to inform social and economic policies, including national responses to the recent COVID-19 pandemic \cite{flaxman2020report, panovska2020determining, kerr2020covasim}. With such critical applications, poor modelling assumptions or software faults can lead to serious repercussions.
% and therefore agent-based models should be scrutinously tested. However, software testing is less prominent in the context of agent-based modelling, perhaps because of the domains in which they are often developed, such as epidemiology and sociology, where few developers have testing experience.

% Software Testing
Software testing is an essential software engineering practice that aims to ensure the quality of software products, including the identification and removal of faults. The time and effort necessary to test software and achieve such quality are significant, often accounting for over 50\% of total project costs \cite{ramler2006economic}. In recent years, a variety of techniques have been proposed to alleviate the cost of testing, from search-based testing \cite{mcminn2004search} to fuzzing \cite{godefroid2008automated}, that automate or partially-automate various testing activities such as the creation of test cases.

% Test Case Generation
Of all software testing activities, perhaps the most labour-intensive and time-consuming activity is the creation of test cases \cite{prasanna2005survey}. As a consequence, the topic of test case generation has received significant attention in recent years, leading to a variety of surveys, techniques and tools supporting the automatic or semi-automatic derivation of test suites \cite{anand2013orchestrated}. However, for many real-world applications, it remains unclear how effective these tools and techniques are, with areas such as scientific software requiring further empirical study to establish their applicability \cite{kanewala2014testing}.

% Agent-Based Models
Agent-based modelling is one area where the applicability of existing test case generation techniques is unclear. Due to their often non-deterministic nature coupled with their complex emergent behaviour, agent-based models present significant challenges for test case generation \cite{russell2002artificial, luck2005agent}. For example, in response to the ongoing COVID-19 pandemic, the UK government has used an agent-based model developed at Imperial College London to inform an economic policy estimated to cost \pounds192.3bn over the 2020-2021 financial year \cite{flaxman2020report, obr2020coronavirus:online}. Despite the importance of testing such critical software, the model contains only basic integration tests configured to a specific set of parameters \cite{mrcideco79:online}. To this end, there have been several recent calls for improved techniques for validation and testing of predictive models \cite{squazzoni2020computational, wynants2020prediction}.

Clearly, there is a need for tools and techniques that make software testing an accessible practice for both researchers and practitioners regardless of their discipline. In this review we aim to identify the current state-of-the-art techniques and future research directions for test case generation in agent-based modelling, paying particular attention to their potential real-world applications. In order to achieve a fair and comprehensive survey of the existing test case generation literature in the agent-based modelling field, this paper reports the results of a systematic literature review in accordance to the guidelines proposed by Kitchenham and Charters \cite{kitchenham2007guidelines}.

The remainder of this work is organised as follows: in Section 2, we provide an overview of agent-based models and test case generation. In Section 3, we present the research methodology including the research questions and review procedure. In Section 4, the results of the systematic literature review are presented, followed by a discussion of some particularly interesting observations in Section 5. In Section 6 we conclude the review and present potential future directions for research.

